Learning to Draw Samples with Amortized Stein Variational Gradient Descent

We propose a simple algorithm to train stochastic neural networks to draw samples from given target distributions for probabilistic inference. Our method is based on iteratively adjusting the neural network parameters so that the output changes along a Stein variational gradient direction (Liu & Wang, 2016) that maximally decreases the KL divergence with the target distribution. Our method works for any target distribution specified by their unnormalized density function, and can train any black-box architectures that are differentiable in terms of the parameters we want to adapt. We demonstrate our method with a number of applications, including variational autoencoder (VAE) with expressive encoders to model complex latent space structures, and hyper-parameter learning of MCMC samplers that allows Bayesian inference to adaptively improve itself when seeing more data.

==> Tex/svgd.tex <==
%!TEX root = ../main.tex
\section{Stein Variational Gradient Descent (SVGD)}
%This proposal will focus on integrating Stein's method with variational inference, by leveraging a new variational interpretation of Stein's characterization \eqref{equ:stein00} discovered in my recent work \citep{liu2016stein}, in which a general purpose inference algorithm called Stein variational gradient descent (SVGD) has been proposed. 
Stein variational gradient descent (SVGD) \citep{liu2016stein} is a general purpose Bayesian inference algorithm motivated by 
Stein's method \citep{stein1972, barbour2005introduction} and kernelized Stein discrepancy \citep{liu2016kernelized, chwialkowski2016kernel, oates2014control}. 
It uses an efficient \emph{deterministic} gradient-based update 
to iteratively evolve a set of particles $\{x_i\}_{i=1}^n$ to minimize the KL divergence with the target distribution. 
SVGD has a simple form that reduces to the typical gradient descent for maximizing $\log p$ when using only one particle $(n=1)$, 
and hence can be easily combined with the successful tricks for gradient optimization, 
including stochastic gradient, adaptive learning rates (such as adagrad), and momentum. % making large scale Bayesian inference both much easier and more efficient. 

To give a quick overview of the main idea of SVGD, let $p(x)$ be a positive density function on $\R^d$ which we want to 
approximate with a set of particles 
$\{ x_i\}_{i=1}^n$. 
SVGD initializes the particles by sampling from some simple distribution $q_0$, and 
updates the particles iteratively by 
%performs iterative updates of form 
\begin{align}\label{equ:xxii}
x_i  \gets x_i +  \epsilon \ff(x_i),  ~~~~ \forall i = 1, \ldots, n,  
\end{align}
where $\epsilon$ is a step size, and 
$\ff(x)$ is a ``particle gradient direction'' %  perturbation direction, or velocity field, 
%which roughly speak, is the gradient of $\KL(q_\vx~||~ p)$ w.r.t. $\vx$, 
chosen to maximumly decrease the KL divergence between the distribution of particles and the target distribution, in the sense that  
%decreases with the fastest speed in the sense that 
\begin{align}\label{equ:ff00}
\ff =   \argmax_{\ff \in \F}  \bigg\{  -   \frac{d}{d\epsilon} \KL(q_{[\epsilon\ff]} ~|| ~ p) \big |_{\epsilon = 0}  \bigg\}, 
%\frac{1}{\epsilon}\{ \KL(q_{t+1}~||~ p )  -  \KL(q_{t}~||~ p) \}, 
\end{align}
where $q_{[\epsilon \ff]}$ denotes the density of the updated particle $x^\prime = x + \epsilon \ff(x) $ when the density of the original particle $x$ is $q$, and $\F$ is the set of perturbation directions that we optimize over. 
We choose $\F$ to be the unit ball of a vector-valued reproducing kernel Hilbert space (RKHS) $\H^d = \H \times \cdots \times \H$ with each $\H$ associating with a positive definite kernel $k(x,x')$; 
%this makes $\F$
%this choice of $\F$ is broad, since $\H^d$
note that $\H$ is dense in the space of continuous functions with universal kernels such as the Gaussian RBF kernel. 
%to allow close approximation of arbitrary continuous functions. 
%which is dense in the space of continuous function with typical non-degenerate kernels such as RBF kernel. 
%We take $\F$ to be the unit ball of a reproducing kernel Hilbert space (RKHS) $\H$ associated with a positive definite kernel $k(x,x^\prime)$, 
%which can be dense in the space of continuous functions with universal (non-degenerate?) kernels such as Gaussian. 
%which is dense in the set of continuous functions when $k(x,x^\prime)$ is non-degenerate \red{(?)},  
%and also makes \eqref{equ:ff00} computationally tractable. 
%{
%{https://papers.nips.cc/paper/4168-universal-kernels-on-non-standard-input-spaces.pdf
%For example, for compact X ? Rd, [30] showed that, among a few others, the RKHSs of the Gaussian RBF kernels are universal, that is, they are dense in the space C(X) of continuous functions f : X ? R. With the help of a standard result from measure theory, see e.g. [1, Theorem 29.14], it is then easy to conclude that these RKHS are also dense in all L1(?) for which ? has a compact support. This key result has been extended in a couple of different directions: For example, [18] establishes universality for more classes of kernels on compact X ? Rd, whereas [32] shows the denseness of the Gaussian RKHSs in L1(?) for all distributions ? on Rd. Finally, [7, 8, 28, 29] show that universal kernels are closely related to so-called characteristic kernels that can be used to distinguish distributions. In addition, all these papers contain sufficient or necessary conditions for universality of kernels on arbitrary compact metric spaces X, and [32] further shows that the compact metric spaces are exactly the compact topological spaces on which there exist universal spaces.
%}

Critically, the gradient of KL divergence in \eqref{equ:ff00} 
equals a simple linear functional of $\ff$, allowing us to obtain a closed form solution for the optimal $\ff$. 
\citet{liu2016stein} showed that 
%A key observation is that the objective in \eqref{equ:ff00} is a linear functional of $\ff$, in fact, we have
\begin{align}\label{equ:klstein00}
&- \frac{d}{d\epsilon} \KL(q_{[\epsilon\ff]} ~|| ~ p) \big |_{\epsilon = 0}  = \E_{x\sim q}[\sumstein_p \ff(x)], \\[.5\baselineskip]
&~~~~\text{with}~~~~~ \sumstein_p \ff(x)  = \nabla_x \log p(x) ^\top \ff (x)+ \nabla_x \cdot \ff(x),  
\end{align}
where $\sumstein_p$ is considered as a linear operator acting on function $\ff$ and is called the Stein operator in connection with Stein's identity which shows that 
the RHS of \eqref{equ:klstein00} equals zero if $p = q$: 
\begin{align}\label{equ:steinid}
\E_{p}[\sumstein_p \ff] =\E_{p}[ \nabla_x \log p ^\top \ff + \nabla_x \cdot \ff] = 0. 
\end{align}
This is a result of integration by parts assuming the value of $p(x)\ff(x)$ vanishes on the boundary of the integration domain.   
%Obviously, $\F$ should be taken as broad as possible, best with infinite dimension, while still allows tractable solution. 
%
%Critically, we show that derivative in \eqref{equ:f00} yields a closed form representation:
%$$  \frac{d}{d\epsilon} \KL(q_{[\epsilon\ff]} ~|| ~ p) \big |_{\epsilon = 0}  = \E_{x\sim q} [\trace(\stein_p \ff(x))], $$Critically, we show that $\F$ to be the unit ball of a reproducing kernel Hilbert space (RKHS) $\H$
%
%
%%$\KL(q_{\vx^t} ~||~ p)$ between the distribution between the distribution $q_{\vx}$ of particles $\vx^t$ and the target distribution decreases with the fastest speed. 
%We take $\F$ to be the unit ball of a reproducing kernel Hilbert space (RKHS) $\H$ associated with positive definite kernel $k(x,x')$. 
%Thanks to an important connection with Stein's identity and kernelized Stein discrepancy, we show that the optimal $\phi$ is given by 
%$\ff(x)$ in RKHS $\H$ associated with positive definite kernel $k(x,x')$, in which case the optimal choice of $\ff(\vx)$ is 

Therefore, the optimization in \eqref{equ:ff00} reduces to 
\begin{align}\label{equ:ksd}
\S(q ~||~ p) \overset{def}{=} \max_{\ff \in \H^d} \{ \E_{x\sim q} [\sumstein_p \ff(x)]  ~~~s.t.~~~~ ||\ff ||_{\H^d} \leq 1\}, 
\end{align}
where $\S(q ~||~ p)$ is the kernelized Stein discrepancy defined in \citet{liu2016kernelized}, which equals zero if and only if $p = q$ under mild regularity conditions. 
Importantly, the optimal solution of \eqref{equ:ksd} yields a closed form% for the optimal solution: of \eqref{equ:ff00}:
 %Further,  it turns out that optimizing \eqref{equ:klstein00} in the unit ball of $\H$ coincides with the variational form of the kernelized Stein discrepancy in \citet{liu2016kernelized},  giving a closed form for the optimal solution of \eqref{equ:ff00}: 
$$
\ff^*(x') \propto  \E_{x\sim q}[\nabla_x \log p(x)k(x,x') + \nabla_x k(x,x')]. 
$$
%This $\ff^*$ can be treated as a gradient of the KL divergence. 
By approximating the expectation under $q$ with the empirical average of the current particles $
\{x_i\}_{i=1}^n$,  SVGD admits a simple form of update: 
\begin{align}\label{equ:update11}
%\begin{split}
%x_i ~ \gets ~ x_i  ~  + ~ \epsilon  \hat\ff^*(x_i) ~~~~~\text{where}~~~~~~ \hat \ff^*(x_i) = \hat \E_{x\in \{x_i\}} [ k(x_i, ~ x) \nabla_{x} \log p(x)  + \nabla_{x} k(x_i, x) ], 
&& &~~~~~~~~~~~ x_i ~ \gets ~ x_i  ~  + ~ \epsilon \Delta x_i, 
~~~~~~~~\forall i = 1, \ldots, n,  \notag
\\
~
&&& \text{where~~~~~}\Delta x_i = \hat \E_{x\in \{x_i\}_{i=1}^n} [  \nabla_{x} \log p(x) k(x, x_i) + \nabla_{x} k(x, x_i) ], 
%x_i ~ \gets ~ x_i  ~  + ~ \epsilon \frac{1}{n} \sum_{x\in \{x_i\}} [ k(x_i, ~ x_j) \nabla_{x} \log p(x)  + \nabla_{x} k(x_i, x) ] . 
%\end{split}
\end{align}
and $\hat\E_{x\sim \{x_i\}_{i=1}^n}[f(x)] = \sum_i f(x_i)/n$. 
The two terms in $\Delta x_i$ play two different roles: 
the term with the gradient $\nabla_x \log p(x)$ drives the particles toward the high probability regions of $p(x)$, 
while the term with $\nabla_x k(x,x_i)$ serves as a repulsive force to encourage diversity;
to see this, consider a stationary kernel $k(x,x') = k(x-x')$, then the second term reduces to $\hat \E_x \nabla_{x} k(x,x_i) = - \hat \E_x \nabla_{x_i} k(x,x_i)$, 
which can be treated as the negative gradient for minimizing the average similarity $\hat \E_x k(x,x_i)$ in terms of $x_i$. 
Overall, this particle update produces diverse points for distributional approximation and uncertainty assessment, and 
also has an interesting ``momentum'' effect in which the particles move collaboratively to escape the local optima.
%See \citet{liu2016stein} for more details. 

It is easy to see from \eqref{equ:update11} that $\Delta x_i$ reduces to the typical gradient $\nabla_x \log p(x_i)$ when there is only a single particle ($n=1$) and $\nabla_x k(x,x_i)$ when $x=x_i$,  
in which case SVGD reduces to the standard gradient ascent for maximizing $\log p(x)$ (i.e., maximum \emph{a posteriori} (MAP)). 

%This update evolves the particles collectively to match the target distribution with the two terms of $\Delta(x_i)$ playing two different roles:    the first term in $\Delta(x_i)$ is theweighted sum of the particles' gradient of the log-density, which drives the particles towards the high probability regions in a collaborative fashion; the second term can be shown to serve as a ``repulsive force'' that makes the particles repel each other to maintain a degree of diversity.
% maintaining a degree of diversity via the second term $\nabla_x k(x_i, x)$ that makes the particles repel each other.

\begin{algorithm}[t]                      % enter the algorithm environment
\caption{Amortized SVGD for Problem~\ref{pro:prob1}}% for Wild Variational Inference}          % give the algorithm a caption
\label{alg:alg1}                           % and a label for \ref{} commands later in the document
\begin{algorithmic}                    % enter the algorithmic environment
\STATE Set batch size $m$, step-size scheme $\{\epsilon_t\}$ and kernel $k(x,x')$. Initialize $\eta^0$. 
\FOR {iteration $t$}
\STATE  Draw random $\{\xi_i\}_{i=1}^m$, calculate $x_i = f(\eta^t;~\xi_i)$, 
and the Stein variational gradient $\Delta x_i$ in \eqref{equ:update11}. 
%\begin{align*}%\label{equ:dxi}
%\Delta x_i = \hat\E_{x\sim\{x_i\}_{i=1}^m} [\log p(x) k(x,x_i) + \nabla_x k(x, x_i)]. 
%\end{align*}
\STATE  Update parameter $\eta$ using \eqref{equ:follow1}, \eqref{equ:follow2} or \eqref{equ:follow3}. 
%$$\eta^{t+1} \gets \eta^{t} + \epsilon ~ \sum_{i=1}^n \partial_\eta f(\eta^t;~\xi_i)  \Delta x_i.$$ 
\ENDFOR
\end{algorithmic}
\end{algorithm}
